Short Range Correlations at Large xbj through Inclusive Electron-nucleus Scattering

The experiment, E08-014, in Hall-A at Jefferson Lab aims to study the short-range correlations (SRC) which are necessary to explain the nuclear strength absent in the mean field theory. The cross sections for $\mathrm{^{2}H}$, $\mathrm{^{3}He}$, $\mathrm{^{4}He}$, $\mathrm{^{12}C}$, $\mathrm{^{40}Ca}$ and $\mathrm{^{48}Ca}$, were measured via inclusive quasielastic electron scattering from these nuclei in a $\mathrm{Q^{2}}$ range between 0.8 and $\mathrm{2.8~(GeV/c)^{2}}$ for $x_{bj}>1$. The cross section ratios of heavy nuclei to $\mathrm{^{2}H}$ were extracted to study two-nucleon SRC for $1<x_{bj}<2$, while the study of three-nucleon SRC was carried out from the cross section ratios of heavy nuclei to $\mathrm{^{3}He}$ for $x_{bj}\ge 2$. Meanwhile, the isospin dependence in SRCs has also been examined through the cross section ratio of $\mathrm{^{48}Ca}$ and $\mathrm{^{40}Ca}$.

==> analysis/backup/analysis_calo.tex <==
\subsection{Electromagetic Calorimeters}

 Energy of scattered electron are completely deposited in Calorimeters after electromagetic the cascade, so the goal of calibration is to relate the ADC signals collected by lead glass blocks in two layers of each Calorimeters to central momentum of scattered electrons (P0). A new variable E/P is defined as a ratio of cluster-reconstructed energy sum of calorimeters and P0, and it should be close to one if ADC channels are well calibrated.


 Due to the difference of two calorimeters, different methods were used to perform the calibrations on each arm. A minimization method was used to calibrate Shower and Preshower\cite{shower_ak}, and the Chi-Square is defined as: 
\begin{equation}
 \chi^{2} = \sum_{i=1}^{N}[\sum_{j\in M_{ps}^{i}}C_{j}\cdot (ADC_{j}^{i}-Ped_{j})+\sum_{k\in M_{sh}^{i}}C_{k}\cdot (ADC_{k}^{i}-Ped_{k})-P_{kin}^{i}]^{2}
\end{equation}

where \emph{i} is the \emph{i-th} event; \emph{j} is the \emph{j-th} preshower block while \emph{k} is the \emph{k-th} shower block;$M_{ps}^{i}$ and $M_{sh}^{i}$ are sets of preshower and shower included in the reconstructed cluster in the \emph{i-th} event; $ADC_{j/k}^{i}$ and $Ped_{j/k}$ respectively represent the ADC channel and mean pedestal value of a preshower or shower block in a certain event \emph{i}; $P_{kin}^{i}$ is the particle momentum in the \emph{i-th} event; and $C_{j/k}$ is a fitting paramter of a block which will be the gain factor of each ADC channel.

 To obtain the best results of fitting, electron samples are selected from data taken at the kinematics region of Quasi-Elastic tail where scattered electrons uniformly distribute along calorimeter blocks. A Fumili minimization package \cite{shower_luhj} is called to minimize the Chi-Square. The improvement after the calibration can be seen from Fig~\ref{pssh_cali}, where electrons are better separated from backgrounds, and  E/P is well centered at one. 

%\clearpage
\parbox[t]{0.45\textwidth}{
 \includegraphics[width=\linewidth]{figures/calo/SH_Calibration.eps}
 \captionof{figure}{\footnotesize{Shower and PreShower calibration}}
 \label{pssh_cali}
}
\hfill
\parbox[t]{0.45\textwidth}{
\includegraphics[width=\linewidth]{figures/calo/PRL_Calibration.eps}
\captionof{figure}{\footnotesize{PRL1 and PRL2 calibration}
\label{prl_cali}}
}

 Similar to the technique of Cherenkov detectors calibration, we aligned the minimum ionization peak in each block of pion rejectors using the cosmic ray data. The advantage of using cosmic ray data for the calibration is that the events uniformly distribut along the detector planes and the energy of particles from cosmic ray, mostly muon, deposited in lead glass blocks should be identical. We located the pedestal peak and muon peak in each ADC spectrum, and align the distance between themto be 100, by applying a gain factor defined as:
\begin{equation}
 C_{i} = \frac{100}{ADC_{i}^{muon}-ADC_{i}^{pedestal}}
\end{equation}

After aligning all ADCs of lead glass blocks, we calculated E/P with new obtained gain factors and did a final correction to shfit the peak to one:
\begin{equation}
 C_{i}^{real} = C_{i} \times \frac{1}{M_{E/P}}
\end{equation}

where $M_{E/P}$ represents the mean value of the E/P peak. The quality of the calibration can be checked from Fig ~\ref{prl_cali}.

 The stability of Calorimeters calibration is checked from Fig~\ref{calo_stability} and resolutions of calibration are extracted. The resolution of calorimeters is 2.53\% per GeV on HRS-R and 3.21\% per GeV on HRS-L, where the one on HRS-L is slightly worse than the one on HRS-R is due to the fact that Pion Rejectors are not total absorbers.

\begin{figure}[ht]
  \includegraphics[width=0.45\linewidth]{figures/calo/R_Calo_Align_new.eps}
  \hfill
  \includegraphics[width=0.45\linewidth]{figures/calo/L_Calo_Align_new.eps}
  \caption{\footnotesize{Calorimeter calibration stability and resolution}}
  \label{calo_stability}
\end{figure}


==> analysis/backup/analysis_cer.tex <==
%\section{Gas Cerenkov}

\subsection{Gas Cerenkov Detectors}

 On both HRS, Gas Cherenkov Detectors (GC) are the main tools to identify pions and electrons. Although pions by design do not directly produce Cherenkov light in the GC, electrons knocked out by pions from gas atoms can fire the detectors and produce signals in the ADC spectra. However, we can identify those signals by considering that their are much weaker than ones produced by scattered electrons. Light radiated by an electron is collected by ten PMTs attached to ten mirrors inside each detector. After ADC channels of each PMT well aligned to represent the same energy scale, the sum of ten ADC signals should be proportional to energy carried by the electron, hence cutting on low values of ADC sum should remove most of pions. We aligned the single photon-electron peak (SPE) of each ADC at around 100 channels by timing a gain factor:
\begin{equation}
 C_{i} = \frac{100}{M_{i}^{SPE}-M_{i}^{pedestal}}
\end{equation}

\begin{figure}[h!]
\includegraphics[width=0.48\linewidth]{figures/cer/Cerenkov_ADC_Align_Before.eps}
\hfill
\includegraphics[width=0.48\linewidth]{figures/cer/Cerenkov_ADC_Align_After.eps}
\caption{\footnotesize{ADC Sum vs Tracking X before and after GC calibration}}
\label{gc_x}
\end{figure}

 where $M_{i}^{SPE}$ and $M_{i}^{pedestal}$ are the mean values of SPE peak and pedestal peak for the $ith$ PMT, fitted by a Gaussian function. The SPE peaks are not significant in our main production triggers ($T1\&T3$), so we perform the calibration with events from T6 and T7 since they do not include GC in the triggers. The improvement of calibration can be demonstrated by Fig~\ref{gc_x}, where the smooth distribution along X axis shows that each ADC is aligned properly. Single photon peaks are aligned to 100 channels after the calibration (Fig~\ref{cer_spe}). The calibration stability was also checked for each momentum setting (Fig~\ref{gc_stability}).

\parbox[t]{0.4\textwidth}{
 \includegraphics[width=\linewidth]{figures/cer/Cer_SPE.eps}
 \captionof{figure}{\footnotesize{GC SPE}}
 \label{cer_spe}
}
\hfill
\parbox[t]{0.5\textwidth}{
 \includegraphics[width=\linewidth]{figures/cer/Cer_SPE_Err.eps}
\captionof{figure}{\footnotesize{Cerenkov SPE vs momentum}}
 \label{gc_stability}
}


==> analysis/backup/analysis_effi.tex <==
\subsection{Efficiencies}

 Detectors are not in 100\% of performance and the inefficiencies of detectors caused by hardware and software are needed to be evaluated corrected for cross section calculation. 

\subsubsection{Trigger Efficiency}

 There are mainly two aspects that determine the trigger efficiency~\cite{R_Bock}, one of which is the trigger algorithm designed to compromize between highly reducing background rate and keeping most of good events, and the other of which would be the dead time caused by electronics and performance of detectors involved in the trigger system. It is important to avoid double counting detectors' inefficiencies when evaluating trigger efficiencies. The definition of trigger efficiency genrally includes the inefficiency of scintillator counters and the formula is writtern as:

\begin{equation}
 \epsilon_{trigger\_eff} = \frac{PS1(3)\times N_{T1(3)}}{PS1(3) \times N_{T1(3)}+PS2(4)\times N_{T2(4)}},
 \label{trigger_eff}
\end{equation}

where $N_{T1(2,3,4)}$ is number of events triggered by T1(2,3,4) after prescaled by PS1(2,3,4). Tranditionally in Hall-A T1(3) is designed by requesting coincidence trigger signals between S1 and S2m, while T2(4) includes signals from GC in the trigger, which should carry the inefficiency effect of GC. However, during the E08014 experiment, T1(3) was modified to include GC signals in trigger, so the detection inefficiency of GC is canceled from the equation. Fig ~\ref{trig_eff} shows that the trigger efficiencies of our data on both arm were better than 99\%.

%\clearpage
\begin{figure}[h!]
\centerline{\includegraphics[width=0.7\linewidth]{figures/scin/Trigger_Eff.eps}}
\caption[Trigger Efficiencies]{\footnotesize{Trigger Efficiencies}}
\label{trig_eff}
\end{figure}

\subsubsection{One-Track Efficiency of VDCs}

Inefficiency of VDCs caused by hardware is neglectable and the majore source is from the misreconstruction of particle tracks during the tracking algorithm. Only one-track events are kept for analysis, and the good events threw away by zero-track and multi-tracks cut are corrected by the one-track efficiency defined as:

\begin{equation}
 \epsilon_{one\_track\_eff} = \frac{N_{Track=1}}{N_{0<=Tracks<=4}}
\end{equation}

 It is very important to select correct electron samples when calculating values of one-track efficiency. We need to avoid applying cuts on variables that require trakcing information, such as variables at focal plane and target plane, and cuting on other VDC variables will introduce other sources of inefficiencies. Cluster-reconstructed variables of calorimeters, such as E/P, can not be used when cutting electrons. cosmic ray events should also be removed since they come with big angles. We could not cut on TOF $\beta$ to suppress cosmic ray background due to the TDC multi-peaks issues on some scintillator bars. During the analysis, we used quasi-elastic carbon data which has low cosmic ray backgound due to the high rates,then applied cut on T1(3) trigger, GC ADC sum and Calorimeters ADC sum to select pure electron events, and we also require only one-hit on each scintillator bar for each event to remove events with multi-particles.From Table~\ref{vdc_table}, we obtained the fraction of one-track and multi-track events, which are above 99\% on each arm.

\begin{table}[h!]
\centering
\begin{tabular}{|c||ccccc|}
	\hline
\textbf{Number of tracks}  & 0 & 1 & 2 & 3 & 4     \\
	\hline \hline
HRS-L   & 0.0298\% & 99.1750\% & 0.7430\% & 0.0452\% & 0.0048\%  \\
        \hline
HRS-R   & 0.0482\% & 99.3600\% & 0.5446\% & 0.0388\% & 0.0073\%  \\
	\hline \hline
\end{tabular}
\caption{Fraction of different tracks events from quasi-elastic data,w/o $\beta$ cut}
\label{vdc_table}	
\end{table}



\subsubsection{Detection Efficiencies of PID detectors}
%\subsubsection{Gas Cherenkov}

For Gas Cherenkov detectors and lead-glass Calorimeters, there are two parts of informations needed to be extracted: the fractions of particles detected when they pass throught the detectors and leave signals, or called detection efficiencies; and the percentages of electrons remaining and pions contaiminating when applying PID cuts, also called PID-Cut efficiencies. PID-Cut efficiencies basically tangle with detection efficiencies due to the fact that we deal with detected events. We need to firstly evalute detection efficiencies and PID-Cut efficiencies will be discussed in next section. 

Detection efficiency of GC (Calorimeters) can be defined as:

\begin{equation}
 \epsilon_{detection\_eff}^{cer(calo)} = \frac{N_{detected}^{cer(calo)}}{N_{samples\_from\_calo(cer)}}
\end{equation}

where $N_{cer(calo)}$ is number of particles detected by GC (Calorimeters), and $N_{samples}$ is number of particle samples from Calorimeters (GC). During the analysis, we cut on T1(3) trigger and spectrometer acceptance, and pure electron were selected by applying cuts on main peaks of E/P spectra of Calorimeters when studying GC, or on the peaks of Cherenkov ADC Sum when studying Calorimeters. 

The design of Hall A Gas Cherenkov detectors should give high detection efficiency, since electrons can easily trigger the detectors with very low threshold, while pions and other particles from cosmic ray can not fire the detectors directly, and the inefficiency is caused by particles hitting the edges of gas boxes or PMT tubes. Fig ~\ref{cer_det_eff} shows that on both arm, the detection efficiencies of Gas Cherenkov detectors are close to 100\%.

%\clearpage
\begin{figure}[h!]
\centerline{\includegraphics[width=0.7\linewidth]{figures/cer/Cer_Det_Eff.eps}}
\caption[Gas Cherenkov Detection Efficiency]{\footnotesize{Gas Cherenkov Detection Efficiency}}
\label{cer_det_eff}
\end{figure}

%\subsubsection{Calorimeters}
The detection efficiencies of lead glass calorimeters are expected to be lower than Gas Cherenkov detectors. Calorimeters are composed by piles of lead glass blocks, so the inefficiency of detection is mainly from particles going through gaps in between blocks or hitting the edges or PMT tubes before cascade. Cluster reconstruction when calculating deposited energy in lead glass blocks is another source of inefficiencies, especially when the electron rate is low and many low energy cosmic ray particles mix in.From Fig ~\ref{calo_det_eff}, we see that the detection efficiencies of calorimeters on both arm are still high than 99\% for most of runs, but for some runs with low electron rates, mainly for $^{3}He$ target with low beam current (Fig~\ref{calo_det_eff_mom}),the detection efficiencies are slightly lower, due to more cosmic ray contamination. Events from cosmic ray will eventually be removed by applying accpetance cuts and PID cuts, so no correction is necessary for those runs.  

\begin{figure}[h!]
 \centerline{\includegraphics[width=0.7\linewidth]{figures/calo/Calo_Det_Eff1.eps}}
 \captionof{figure}{\footnotesize{Calorimeters: Efficiencies vs Run Number}}
 \label{calo_det_eff}
\end{figure}

\begin{figure}[h!]
 \centerline{\includegraphics[width=0.7\linewidth]{figures/calo/Calo_Det_Eff_Mom1.eps}}
 \captionof{figure}{\footnotesize{Calorimeters: Efficiency vs Momentum}}
 \label{calo_det_eff_mom}
\end{figure}

==> analysis/backup/analysis_pid.tex <==
\subsection{Particle Indentification}
 
 The goal of cuts efficiency study is to obtain most optimized cut values on PID detectors to reject most of background particles (mainly pions) while keeping as more electrons as possible. The kinematic settings of E08014 experiemnt determine that the production of pions is much rare comparing with scattered electrons, and the new trigger design also has already removed most of pions during online data taking by intruducing GC detectors in the trigger system, so we are supposed to have high cut efficiencies and very small pions contamination. 
 
 Events from T6 and T7 triggers were used to study the PID cut efficiencies since they contain more pions. Acceptance cuts and VDCs One-Track cuts were also applied to eliminate cosmic ray events and multi-scattering electrons. Then pure pion samples and pure electrons samples were chosed from Calorimeters (GC) when we studied cut efficiency of GC (Calorimeters). The percentages of pions and electrons left over after cutting GC (Calorimeters) are called pion rejection efficiency and electron cut efficiency, respectively, and the definitions are given by:

\begin{equation}
 \epsilon_{pion\_rej}^{cer(calo)} = \frac{N_{pion\_after\_cut}^{cer(calo)}}{N_{pion\_samples\_from\_calo(cer)}},  \epsilon_{electron\_cut}^{cer(calo)} = \frac{N_{electron\_after\_cut}^{cer(calo)}}{N_{electron\_samples\_from\_calo(cer)}},     
    \end{equation}


 A procedure of cut scanning is to obtain pion rejection efficiency and electron cut efficiency, then to determine most suitable cut values. Fig~\ref{Lgc_eff} and Fig~\ref{Rgc_eff} shows that cutting on low channels (50) of GC ADC sum can already remove most of pions while keep more than 99\% of electrons. The combination  cuts on E/P (0.5 on both arms) and the second layer ADC sum of Calorimeters (100 for PRL2 and 200 for Shower) will further remove above 90\% of pions while still above 99\% of electrons remaining (Fig~\ref{Lcalo_eff} and Fig~\ref{Rcalo_eff}). Totally for data in HRS-L and HRS-R, 99.85\% (99.62\%) of pions are eliminated with PID cuts, and meanwhile, 99.58\% and 99.86\% of electrons surivive after the cuts. Considering the high electrons rates and low pion production for our kinematics, we don't need special corrections of pion contaimination.

\begin{figure}[h!]
\centerline{\includegraphics[width=0.8\linewidth]{figures/pid/L_Cer_PID_Cut.eps}}
\caption[GC cut efficiencies on HRS-L]{\footnotesize{GC cut efficiencies on HRS-L}}
\label{Lgc_eff}
\end{figure}

\begin{figure}[h!]
\centerline{\includegraphics[width=0.8\linewidth]{figures/pid/R_Cer_PID_Cut.eps}}
\caption[GC cut efficiencies on HRS-R]{\footnotesize{GC cut efficiencies on HRS-R}}
\label{Rgc_eff}
\end{figure}

\begin{figure}[h!]
\centerline{\includegraphics[width=0.8\linewidth]{figures/pid/L_Calo_PID_Cut.eps}}
\caption[Calorimeters cut efficiency on HRS-L]{\footnotesize{Calorimeters cut efficiency on HRS-L}}
\label{Lcalo_eff}
\end{figure}

\begin{figure}[h!]
\centerline{\includegraphics[width=0.8\linewidth]{figures/pid/R_Calo_PID_Cut.eps}}
\caption[Calorimeters cut efficiency on HRS-R]{\footnotesize{Calorimeters cut efficiency on HRS-R}}
\label{Rcalo_eff}
\end{figure}

As we discuss in the previous section, values of cut efficiencies should be corrected by detection efficiencies of the detectors since pion and electron samples from other detectors are not necessarily detected by the detectors due to their inefficiencies. Because detection efficiencies don't relate to particle types, pion rejection efficiency and electron cut efficiency should correctly redefined as:
 
\begin{equation}
 \epsilon_{pion\_rej}^{cer(calo)} = \frac{N_{pion\_after\_cut}^{cer(calo)} \cdot \epsilon_{det}^{cer(calo)}}{N_{pion\_samples\_from\_calo(cer)}},  \epsilon_{electron\_cut}^{cer(calo)} = \frac{N_{electron\_after\_cut}^{cer(calo)} \cdot \epsilon_{det}^{cer(calo)}}{N_{electron\_samples\_from\_calo(cer)}},        
\end{equation}

 The detection efficiencies of PID detectors in Hall-A are near 99.9\% as we discussed in the previous section so we don't correct the values of PID cut efficiencies. 

==> intro/backup/intro.tex <==
\chapter{Physics Motivation}
 Understanding the structure of the nucleus remains as one of the biggest challenges in nuclear physics because of the complicated many-body interaction between nucleons. The independent particle shell model has its great success in description of the nuclear structure as individual nucleons moving in the average mean field, and their energy and momenta are below the Fermi energy and the Fermi momentum, i.e., $\epsilon < \epsilon_{F}$ and $k<k_{F}$. However, the theory provides limited ability to study the short range properties of nucleon-nucleon (NN) interaction and fails to describe the structure of nuclear matter beyond the saturation density. 
 
 Short Range Correlations (SRCs) provide an successful explanation of such discrepancy by examining the high momentum component of the nucleon momentum distribution at $k>k_{F}$. The attractive and repulsive potential between nucleons at short distance ($\sim 1.0$ fm) excite the nucleons from their single shell and cause the significant increase of strength to the nuclear spectral function. 

High energy electrons scattering on a nuclear target provides an essential probe to unveil the tiny structure of nuclei and nucleons. In the kinematic region of quasi-elastic (QE) scattering, the electron interacts with the target by exchanging a virtual photon which is able to couple to a meson exchanged between two nucleons. The measurement of such process is able to resolve the nucleon-nucleon (NN) interaction and provide an effective way to study the structure of nuclear. Early experiments in SLAC conformed the evidence of SRCs and recent experiments in JLab extended the study to map out the strength of SRCs in a wider range of nuclei and examined the isospin effect in SRCs. 

 In this chapter, a review of QE electron-nucleus scattering will be given in Section 1.1, followed by a discussion of theoretical understandings of nuclear properties including the IPSM in Section 1.2 and SRCs in Section~1.3. The experimental techniques and results to explore SRCs will be briefly reviewed, and the new experiment, E08-014, will be introduced at the end.

\input intro/qe.tex
\input intro/nuclear_structure.tex
\input intro/src.tex


==> intro/backup/nuclear_structure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Overview
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Independent Particle Shell Model}
A nucleus is a tiny object with its typical size of about 1.2~fm, which, however, is a complicated many-body system where nucleons are bound by strong interactions. To fully understand the detailed structure of the nucleus, one needs to have the complete knowledge of each nucleons' eigen-state. For a light nucleus with only few nucleons, the wave functions can be directly calculated using variational methods~\cite{PhysRevLett.87.172502}. However, for medium and heavy nuclei ($A\geq 12$), the explosion of degree of freedom in the Hamiltonian makes it impossible to obtain the solution.
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/CentralTensorFull}
    \caption[Two-nucleon potential distribution]{\footnotesize{Two-nucleon potential distribution \cite{donal_prvt}, where the blue line represents the tensor force which responds most of the attractive part.}}
    \label{potential_well}Compared with the general size of an atom, a
  \end{center}
\end{figure}

Furthermore, the particular behaviour of the interaction potential between nucleons also increases the complexity of the nuclear system. As shown in Fig.~\ref{potential_well}, two nucleons experience weak attractive interaction at moderate distance. As they get closer, the strong attractive force, mainly caused by the tensor components of spin and isospin channels, forms a deep potential well. At much short distance, the hard-core interaction between nucleons generates strong repulsion which prevents the nucleus from further collapses. The Coulomb force between protons and potential three-body forces also play a role but they are much weaker compared with the strong force.

Despite the complexity of the nucleus, Scattering experiment observed the spectroscopes of nucleons which reveal that nucleons behave more like independent particles in nuclear medium due to the collective effects of Pauli principle and the strong short-distant interactions with surrounding nucleons. Nucleons occupy different energy shells similar to the arrangement of electrons orbiting around the nucleus. 

The explanation of these phenomena has been successfully approached by independent particle shell model, in early circumstance also called as the mean field theory. In this theory, the nucleus is treated as a non-relativistic object where nucleons interact only through two-body interaction. Nucleons tend to occupy the lowest energy state first and the energy of the last occupied state is called the Fermi energy. The whole set of occupied energy levels is called the Fermi sea. Combined with the spin-orbit coupling, IPSM successfully predicts the ground state properties, the excitation of nuclei at low energy, nuclear spins and parities, as well as the prediction of nuclear magic numbers. However, IPSM shows its limitation in predicting the nuclear magnet moments and highly excited energy states. 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.50\linewidth]{./figures/physics/spec_fac_exp}
    \caption[Experiment measurements of spectroscopy factors]{\footnotesize{Experiment measurements of spectroscopy factors for different nuclei deviate from one, indicating the important role of correlations between nucleons.}}
    \label{spec_fac_exp}
  \end{center}
\end{figure} 

A useful experimental observable, called Spectroscopy Factor, denotes the amplitudes of adding or removing one nucleon from the nucleus. In IPSM, assuming nucleons occupy $j$ orbits in the nuclear shell, the cross section of removing one nucleon is then written as, $\sigma_{removing} = S\cdot\sigma_{sp}$, where $\sigma_{sp}$ is the single-particle cross section, and the spectroscopy factor, $S$, should obey a sum role:
\begin{equation}
  \frac{S}{(2j+1)} \equiv 1,
\end{equation} 
where the factor $(2j+1)$ denotes the maximum energy states of the nucleon. Several measurements ~\cite{Lapikas1993297,Kelly:1996hd} with medium-energy proton-knock experiments in early 1970s measured the values of spectroscopy factor for heavy nuclei (Fig.~\ref{spec_fac_exp}) which is $30\%-40\%$ lower than one. Even advanced Hartree-Fock calculations~\cite{hartree_fock_book} involving long range nucleon-nucleon interaction still overestimate the nuclear strength.


==> intro/backup/qe.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\chapter{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%High energy electrons scattering on a nuclear target provides an essential probe to unveil the tiny structure of nuclei and nucleons. The electron interacts with the target by exchanging a virtual photon which includes both the longitudinal and transverse components, comparing with the transversely polarized real photon. In the kinematic region of quasi-elastic (QE) scattering, the virtual photon is able to couple to a meson which is exchanged between two nucleons. The measurement of such process is able to resolve the nucleon-nucleon (NN) interaction and provide an effective way to study the structure of nuclear as discussed in next chapter.

% In this chapter, a review of QE electron-nucleus scattering will be given, followed by a discussion of extracting the spectral function and the momentum distribution of the knock-out nucleon via the inclusive cross sections measurement.

\section{Electron-Nucleus Quasi-elastic Scattering}
\begin{figure}[!ht]
  \begin{center}         
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/e_scatt}
    \caption[Schematic of electron-scattering on a nucleus]{\footnotesize{Schematic of electron-scattering on a nucleus}}
    \label{e_scatt}
  \end{center}
\end{figure}
An electron with predefined initial energy and final energy, $E_{e}$ and $E'_{e}$, interacts with a charged nucleus by exchanging a virtual photon with the energy transfer, $\nu = E_{e}-E'_{e}$ (Fig.~\ref{e_scatt}). By varying the amplitude of the energy transfer, one can probe the nucleus at different scales. At low energy transfer, electrons interact with the entire nucleus and the measurement of elastic cross section is generally applied in the study of nuclei and nucleons form factors~\cite{bfrois}. 

As shown in Fig.~\ref{e_trans}~\cite{qe_donal}, a process of quasi-elastic (QE) electron-nucleon scattering appears with larger energy transfer, and the Fermi motion of the nucleon in the nucleus results an broad distribution compared to the shape elastic peak. Nucleons are excited at even larger energy transfer and resonances start to contribute to the cross section. 

Electrons directly probe the quarks properties at very large energy transfer through the process of deep inelastic scattering (DIS). 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/eesm}
    \caption[Electron energy transfer]{\footnotesize{Inclusive cross section on the y-axis versus the energy loss,$\omega=\nu=E_{e}-E'_{e}$, on the x-axis.}}
    \label{e_trans}
  \end{center}
\end{figure}

A convenient parameter for identifying different processes in the scattering is the Bjorken variable, $x_{bj}=Q^{2}/(2m_{N}\nu)$, where $m_{N}$ is the nucleon mass. The original definition of $x_{bj}$ is the momentum fraction of the quark constituents from the nucleon during the DIS scattering. In electron-nucleon scattering, the elastic peak locates at $x_{bj}=1$, while for inelastic process, $0<x_{bj}<1$. In electron-nucleus scattering, $x_{bj}$ extends to the region of $0<x_{bj}<M_{A}/m_{N}$, $x_{bj}=1$ is now the location of the quasi-elastic peak, and the elastic peak moves to $x_{bj}=M_{A}/m_{N}$. For convenience, $m_{N}$ is usually replaced by the proton mass during the experimental data analysis, as used in the rest of this thesis:
\begin{equation}
  x_{bj} = Q^{2}/(2m_{p}\nu).
  \label{xbj_define}
\end{equation}  

During the quasi-elastic scattering, an electron knocks a nucleon out from the nucleus (Fig.~\ref{e_scatt}), which provides a opportunity to study the property of nuclear structure. In the picture of plane-wave impulse approximation (PWIA), the exclusive electron scattering cross section is the sum of the cross sections of the individual nucleons as:~\cite{john_thesis}:
\begin{equation}
  \frac{d^{5}\sigma}{dE'_{e}d\Omega_{e} d^{3}\vec{p'}} = \sum_{nucleons}\sigma_{eN}\cdot S'_{N}(E_{0},\vec{p}_{0}),
  \label{quasi_xs_spectral_function}
\end{equation}
where $S'_{N}(E_{0},\vec{p}_{0})$, called the nuclear spectral function, is the probability of removing a nucleon with initial energy $E_{0}$,  and momentum $\vec{p}_{0}$ from the target nucleus~\cite{qe_donal}, and $\sigma_{eN}$ is the electron-nucleus cross section. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 	  
\subsection{Inclusive Cross Section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 	  
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/includ_diagram}
    \caption[Schematic of inclusive QE electron scattering]{\footnotesize{Schematic of inclusive QE electron scattering where $\vec{p}_{A-1} = -\vec{p}_{0}$ for fixed targets.}}
    \label{includ_scatt_diag}
  \end{center}
\end{figure}
As shown in Fig.~\ref{includ_scatt_diag}, the inclusive electron scattering cross section is measured by only detecting the scattered electrons ($\sqrt{M^{2}+ \vec{p}^{2}}$, $\vec{p}$), while the final state of the ($A-1$) recoil system,($\sqrt{M_{A-1}^{2}+ \vec{p}_{A-1}^{2}}$, $\vec{p}_{A-1}$), remains unknown. To obtain the inclusive cross section from Eq~\eqref{quasi_xs_spectral_function}, one separates the contributions from protons and neutrons, and integrates over the final states of the nucleons:
\begin{equation}
  \frac{d^{3}\sigma}{dE'd\Omega} = \int (Z\sigma_{ep}S'_{p}(E_{0},\vec{p}_{0})+N\sigma_{en}S'_{n}(E_{0},\vec{p}_{0})) d^{3}\vec{p},
\end{equation}
where the subscripts in $dE'_{e}d\Omega_{e}$ have been omitted since only electrons are measured.

Assuming the spectral function is spherically symmetric, and if the difference in the spectral function between protons and neutrons is ignored, the more general form $S'(E_{0},p_{0})$ can be factored out from the equation. Since $\vec{p} = \vec{p}_{0}+\vec{q}$, where $\vec{q}$ is fixed when measuring $E_{0}$ and $E'$, one can replace $d^{3}\vec{p}$ by $d^{3}\vec{p}_{0}$. In the spherical coordinate, $d^{3}\vec{p}_{0}=p_{0}^{2} dp_{0}d(cos\theta) d\phi$, and the cross section becomes:
\begin{equation}
  \frac{d^{3}\sigma}{dE'd\Omega} = 2\pi \int \tilde{\sigma}_{0}\cdot S'(E_{0},p_{0})\cdot p_{0}^{2}dp_{0}d(cos\theta)
  \label{in_xs_org}
\end{equation}
where
\begin{equation}
  \tilde{\sigma}_{0} = \frac{1}{2\pi}\int_{0}^{2\pi} \left( Z\sigma_{ep}+N\sigma_{en} \right)d\phi.
\end{equation}

Eq~\eqref{in_xs_org} can be further simplified by considering the energy conservation. From Fig.~\ref{includ_scatt_diag}, for the fixed target, $\vec{p}_{A-1} = - \vec{p}_{0}$, which gives: 
\begin{equation}
  M_{A}= E_{0}+ \sqrt{M_{A-1}^{*2}+p_{0}^{2}},
\end{equation}
and,
\begin{equation}
  \quad  M_{A}+\nu = \sqrt{M^{2}+(\vec{p}_{0}^{2}+\vec{q}^{2})}+\sqrt{M_{A-1}^{*2}+\vec{p}_{0}^{2}},
  \label{ene_mom_cons}
\end{equation}
where $M$, and $M_{A}$ are the mass of the ejected nucleon and the target nucleus, respectively. $M_{A-1}^{*}$ is the mass of the recoiling $(A-1)$ system, where the superscript * means it could be in its excited state. Eq~\ref{in_xs_org} becomes~\cite{john_thesis}:
\begin{equation}
  \frac{d^{3}\sigma}{dE'd\Omega} = 2\pi \int \tilde{\sigma}_{0}\cdot \frac{E_{N}}{|\vec{p}_{0}||\vec{q}|} \cdot S'(E_{0},p_{0})\cdot p_{0}^{2}dp_{0}dE_{0}
\end{equation}
where $E_{N}=\sqrt{M^{2}+\vec{p}}$ denotes the energy of the struck nucleon.

One can define the separation energy, $E_{s}\equiv M_{A-1}^{*}+M-M_{A}$. Then the spectral function becomes $S(E_{s},p_{0})\equiv - S'(E_{0},p_{0})$, where the Jacobian transformation factor from $E_{0}$ to $E_{s}$ has been absorbed into the new definition~\cite{john_thesis}. One can define $\tilde{\sigma}=\tilde{\sigma_{0}}\cdot E_{N}/|\vec{q}|$, and rewrite the cross section as:
\begin{equation}
  \frac{d^{3}\sigma}{dE'd\Omega} = 2\pi \int_{E_{s}^{min}}^{E_{s}^{max}} \int_{p_{0}^{min}}^{p_{0}^{max}}\tilde{\sigma}\cdot S(E_{s},p_{0})\cdot p_{0}dp_{0}dE_{s},
  \label{in_qe_xs1}
\end{equation}
where $p_{0}^{min}$ and $p_{0}^{max}$ are the solution of Eq~\eqref{ene_mom_cons} when $\vec{p}_{0}$ and $\vec{q}$ are parallel:
\begin{equation}
  \quad  M_{A}+\nu = \sqrt{M^{2}+y^{2}+2yq+q^{2}}+\sqrt{M_{A-1}^{*2}+y^{2}},
  \label{ene_mom_cons_y}
\end{equation}	
where two solutions, $y_{1}$ and $y_{2}$ ($y_{1}<y_{2}$), give the values of $p_{0}^{min}$ and $p_{0}^{max}$, respectively. While $E_{s}^{min}$ corresponds to the minimum separation energy when the recoil nucleus is in its ground state, $E_{s}^{max}$ is the maximum separation energy when the struck nucleon is at rest:
\begin{equation}
  E_{s}^{max}=\sqrt{(M_{A}+\nu)^{2}-q^{2}}-M_{A}.
\end{equation}
which leads to $p_{0}^{min}(E_{s}^{max}) = p_{0}^{max}(E_{s}^{max})$.

\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/pkem}
    \caption[Spectral Function]{\footnotesize{Spectral Function versus separation energy $E_{s}$ and transfer momentum $p_{0}$~\cite{qe_donal}.}}
    \label{pkem}
  \end{center}
\end{figure}
Because the spectral function decreases rapidly by orders of magnitude toward $E_{s}^{max}$ and $p_{0}^{max}$, see Fig.~\ref{pkem}, the upper limits of the two integrals in Eq~\eqref{in_qe_xs1} can be extended to infinity. Meanwhile, $\tilde{\sigma}$ changes very slow as a function of $E_{s}$ and $p_{0}$ so can be factored out from the integral and evaluated at the maximum value of the spectral function at $E_{s}=E_{s}^{0}$. Hence Eq~\eqref{in_qe_xs1} can be rewritten as:
\begin{equation}
  \frac{d^{3}\sigma}{dE'd\Omega} = 2\pi \bar{\sigma}\int_{E_{s}^{min}}^{\infty} \int_{p_{0}^{min}}^{\infty}S(E_{s},p_{0})\cdot p_{0}dp_{0}dE_{s},
  \label{in_qe_xs2}
\end{equation}
where $\bar{\sigma} \propto \tilde{\sigma}(E_{s}^{0},p_{0}^{min})$~\cite{PhysRevB.36.1208}. The model of $\bar{\sigma}$ is usually taken from the prescription by De Forest~\cite{DeForest1983}, shown as~\cite{john_thesis}:
\begin{equation}
  \bar{\sigma} = \frac{1}{Z\sigma_{p}+N\sigma_{n}}\frac{|\vec{q}|}{\sqrt{M^{2}+(y+\vec{q})^{2}}}.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Momentum Distribution and y-Scaling}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 	  
The integral of the spectral function over the separation energy leads to the momentum distribution:
\begin{equation}
  n(p_{0}) = \int_{E_{s}^{min}}^{\infty} S(E_{s},p_{0})dE_{s},
  \label{np_mom_eq}
\end{equation}
which is a sensitive probe to examine the effect of the nuclear medium and nucleon-nucleon interactions. At momenta above the Fermi momentum, $k_{F}$, the mean field effect vanishes and strong short range correlations of the nucleons emerge.

The spectral function is directly connected to the momentum distribution, but it is not an experimental observable. Instead, one can examine the scaling behavior~\cite{West1975263} of inclusive quasielastic scattering cross section. The scaling function can be defined as~\cite{PhysRevC.41.R2474,Boffi19931}:
\begin{equation}
  F(y,q) = 2\pi\int_{E_{s}^{min}}^{\infty} \int_{|y|}^{\infty}S(E_{s},p_{0})\cdot p_{0}dp_{0}dE_{s}.
  \label{fy_scaling_eq}
\end{equation}
where the new variable, $y$, is defined as the minimum values of momentum in Eq~\eqref{ene_mom_cons}, $p_{0}^{min}=|y|$, when the $A-1$ system is in its ground state:
\begin{equation}
  M_{A}+\nu = \sqrt{M^{2}+q^{2}+y^{2}+2yq}+\sqrt{M_{A-1}^{2}+y^{2}}.
  \label{y_enegy_conserv}
\end{equation} 
If only the nucleonic degrees of freedom are considered, the scaling function becomes independent of $\vec{q}$ at large momentum transfer~\cite{Boffi19931}. Hence, $F(y,q)\equiv F(y)$. From Eq~\eqref{in_qe_xs2}, the scaling function can be extracted from electron-nucleon scattering cross section for an off-shell nucleon:
\begin{equation}
  F(y)=\frac{d^{3}\sigma}{dE' d\Omega } \frac{1}{Z\sigma_{p}+N\sigma_{n}} \frac{q}{\sqrt{M^{2}+(y+q)^{2}}}.
  \label{fy_scaling_eq2}
\end{equation}
Due to the Fermi motion, the broad quasielastic peak of the inclusive cross section is mixed with the tails of resonance and DIS components, as shown in Fig.~\ref{e_trans}. To extract $F(y)$ from the experimental cross section, one needs to utilize a cross section model to remove the contribution from DIS region, $\sigma_{QE}=\sigma_{Exp}-\sigma_{DIS}^{model}$ (See Appendix B).

By reversing the order of the integration in Eq~\ref{fy_scaling_eq} and based on Eq~\eqref{np_mom_eq}, $F(y)$ can be rewritten as:
\begin{equation}
  F(y) = 2\pi\int_{|y|}^{\infty}n(p_{0})\cdot p_{0}dp_{0}.
  \label{fy_mom_eq}
\end{equation} 
Hence the momentum distribution can be extracted experimentally by measuring the $F(y)$ distribution~\cite{qe_donal}:
\begin{equation}
  n(p_{0}) = \frac{-1}{2\pi p_{0}}\frac{dF(p_{0})}{dp_{0}} \mid_{p_{0}=|y|},
  \label{mom_dis_fy}
\end{equation}
The scaling of $F(y)$ is supposed to be valid in the limit of very large momentum transfer where the effects due to final-state interactions and the error made by extending the upper limit of Eq~\eqref{fy_mom_eq} to infinity can be neglected. Meanwhile, the assumption that the lower limit ($p_{0}^{min}=|y|$) is independent of $E_{s}$ is also needed to be verified. The momentum distribution can be extracted from data in the scaling region, but the data in the region of approaching to scaling is also important to verify those assumptions.


==> intro/backup/src.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SRCs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Short Range Correlations in Nuclei}
To understand why the mean field theory fails to predict the nuclear strength and how SRCs attribute to the explanation of the missing nuclear strength, one needs to examine the modern nucleon momentum distributions which directly relate to the nucleon properties in the nucleus. While the prediction of mean field theory gives a rapid fail-off curve at momenta approaching $k_{F}$, shown in Fig.~\ref{mom_dis_ox}, experimental results~\cite{PhysRevC.53.1689} present the momentum tail with much slow falloff at $k>k_{F}$ which is similar for all nuclei from deuterium to nuclear matter. The results strongly argues again the mean field prediction, but can be easily understood if the high momentum tails are generated by the short-range part of NN interactions, i.e., SRCs.

From Fig.~\ref{potential_well}, nucleons interact at very short distance via the attractive potential which is mainly contributed by the tensor force, but their strong repulsive hard-cores prevents them to further collapse. Such dramatic processes create a correlated configuration with large relative momenta. The excitation of nucleons from these configurations significantly increase the momentum strength at $k>k_{F}$ which is not predicted by the mean field theory. However, the excitations are not related to any real excited statues of the nucleus since the total momentum of the correlated nucleons is relatively small. 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.80\linewidth]{./figures/physics/Claudio_Distributions}
    \caption[Nucleon momentum distribution]{\footnotesize{Nucleon momentum distribution for various nuclei~\cite{PhysRevC.53.1689}, where dotted lines are from a mean field calculation, solid lines are from calculations involving SRCs. Dots are from experimental data.}}
    \label{mom_dis_ox}
  \end{center}
\end{figure}

In the picture of SRCs, the asymptotic form of momentum distribution can be broke down into several regions. At $k\leq k_{F}$, the strength is mainly contributed by the mean field potential. At the momentum range \emph{300 $<$ $k$ $<$ 600} MeV/c, the contribution of the mean field effect vanishes and the effect of two-nucleon short range correlation (2N-SRC) becomes dominant. The nucleons in this configuration carry large and back-to-back momenta, while the total momentum of the NN pair is negligible. Due to the fact that the NN attraction is dominated by the tensor components which produce iso-singlet pairs, i.e., $(np)_{I=0}$, one expects to see the high momentum tails of heavy nuclei to be identical to the one of deuteron, as shown in Fig.~\ref{mom_dis_ox}. The configuration of 2N-SRC breaks down at much higher momentum limit (\emph{600 $\leq$ $k$ $\leq$ 800} MeV/c) where the isospin-independent repulsive core begins to dominate, and the inclusion of three-nucleon short range correlation (3N-SRC) should be manifested~\cite{src_john}. At extremely high $k$ limit where the nucleon kinetic energy is comparable with the excitation energy of nucleons, non-nucleonic degree-of-freedom may be needed to be considered~\cite{src_john}.
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.80\linewidth]{./figures/physics/2NSRC3NSRC}
    \caption[Diagrams of 2N- and 3N-SRC]{\footnotesize{Diagram of 2N- and 3N-SRC. On the left diagram the virtual phone breaks up the 2N-SRC pair in back-to-back ejection, and on the right diagram the break-up of 3N-SRC configuration results in correlated nucleon ejecting in different direction so their total momentum remains at zero.}}
    \label{2nsrc3nsrc}
  \end{center}
\end{figure}

\subsection{Two-Nucleon Correlations}
Based on the discussion above, the dominance of 2N-SRC in the nucleus at $k>k_{F}$ should yield an momentum distribution proportional to the one in deuterium:
\begin{equation}
  n_{A}(k) = a_{2}(A,Z)\cdot n_{D}(k), \qquad for\quad k>k_{F},
  \label{2nsrc_mon_scaling}
\end{equation}   
where $n_{D}(k)$ denotes the momentum distribution of deuterium and $a_{2}(A,Z)$ relates to the probability of finding such two-nucleon configuration in the nucleus with nuclear number $A$ and proton number $Z$. One can study the scaling of $a_{2}$ as the function of \emph{k}, by taking ratio of momentum distribution of different nuclei to deuterium, $n_{A}(k)/n_{D}(k)$.

The momentum distribution can be reconstructed from the ground state wave-function but is not an experimental observable. Instead, one studies SRCs through the spectral function which directly relates to the cross section of physical processes (Eq~\ref{quasi_xs_spectral_function}). In IPSM, one can define the spectral function as~\cite{Frankfurt_misak}:
\begin{equation}
  S_{A}(E_{R},p_{i}) = |<\phi_{A-1}|\delta(-p_{i}^{2}/(2m_{A-1}) + E_{R}-E_{m})a(k)|\psi_{A}>|^{2}, 
  \label{spectral_2nsrc}
\end{equation}
which represents a product of the probability of finding a nucleon in the nucleus with initial momentum $p_{i}$, and the probability of the residual system carrying recoil energy $E_{R}$ after the removal of this nucleon. \emph{a(k)} denotes an operator to remove a nucleon from the nucleus A, $E_{m}$ depends on A and represents the excitation energy of the $A-1$ system at rest, and $-p_{i}^{2}/(2m_{A-1})$ is the kinetic energy of the center of mass. 

When a nucleon in the 2N-SRC configuration is instantly knocked out by a high energy probe, its paired nucleon with an equal momentum is rejected in the opposite direction, while the $A-2$ residual nucleus remains unperturbed ($E_{m}\sim 0$). When only the knock-out nucleon is interested, the kinetic energy of the correlated nucleon is shared by the entire $A-1$ system. From Eq~\eqref{spectral_2nsrc}, the average recoil energy of the $A-1$ system can be approximately given as:
\begin{equation}
  <E_{R}>_{2N-SRC} \sim \frac{p^{2}_{i}}{2m_{N}}.
  \label{Er_2nsrc}
\end{equation}

Since $E_{R}$ directly relates to the initial momentum of the nucleon in 2N-SRC, and the spectral function links to the momentum distribution (Eq.~\eqref{np_mom_eq}), observation of the correlation between the spectral function and $E_{R}$ enables one to examine the contribution of SRCs but however, it is not uniquely sensitive to SRCs. Indeed, any processes that involving NN interaction, such as meson exchange currents,yields the same result in Eq~\eqref{Er_2nsrc}. One can check the dominance of the SRCs by applying additional kinematic conditions to suppress long range NN interactions, which will be discussed in next section.

\subsection{Three-Nucleon Correlations}
Similar to the deuterium-like configuration of the 2N-SRC pair, the momentum distribution of a nucleon in a 3N-SRC configuration should be identical to the case in $^{3}H$ (pnn) and $^{3}He$ (ppn). For example,
\begin{equation}
  n_{A}(k) = a_{3}(A,Z)\cdot n_{^{3}He}(k), \qquad for\quad k>800 \quad MeV/c,
  \label{3nsrc_mon_scaling}
\end{equation}  
where similarly, $n_{^{3}He}(k)$ is the momentum distribution of $^{3}He$ and $a_{3}(A,Z)$ is the probability of finding three-nucleon configuration in the nucleus $A$. 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.80\linewidth]{./figures/physics/3nsrc_two_types}
    \caption[Two types of 3N-SRC configuration]{\footnotesize{Two types of 3N-SRC configuration~\cite{Frankfurt_misak}.}}
    \label{3nsrc_two_types}
  \end{center}
\end{figure}

However, the configuration of 3N-SRC is more complicated compared with the simple back-to-back picture of 2N-SRC. In general, there are two types of 3N-SRC, as shown in Fig.~\ref{3nsrc_two_types}. The first type, namely 3N-SRC-I, is the situation of two nucleons share the initial momentum which is equal to the struck nucleon but in the opposite direction, a configuration similar to 2N-SRC but involving three nucleons. The effect of 3N-SRC-I typically dominates at $p_{i}\geq 600 MeV/c$ with the average recoil energy of the $A-2$ residual system:
\begin{equation}
  <E_{R}>_{3N-SRC-I} \sim \frac{p^{2}_{i}}{4m_{N}}.
  \label{Er_3nsrc_1}
\end{equation}
which is approximately equal to one half of the recoil energy in 2N-SRC. This configuration gives the major contribution in the kinematic region of 3N-SRC.

The second type, 3N-SRC-II, refers to the configuration of three nucleon carrying momenta all exceeding the Fermi momentum in three different direction, and the average recoil energy of the residual system in this configuration is:
\begin{equation}
  <E_{R}>_{3N-SRC-II} \sim \frac{p^{2}_{i}}{m_{N}},
  \label{Er_3nsrc_2}
\end{equation}
which is larger than the average recoil energy of 3N-SRC-I, indicating the probability of 3N-SRC-II is more rare than the one of 3N-SRC-I, although the former one is easier to be observed experimentally. 

Eq~\eqref{Er_2nsrc}, Eq~\eqref{Er_3nsrc_1} and Eq~\eqref{Er_3nsrc_2} reveal that the average recoil energy of 2N-SRC is in between the two average recoil energies of 3N-SRC, and for 2N-SRC the distribution of $E_{R}$ as a function of $p_{i}$ is very broad, so its capability of identifying contributions from 2N-SRC and 3N-SRC to the spectral function is limited. New kinematic quantities are needed to separate these two processes, and are introduced next.

\subsection{Relativistic Approach}
The high energy process of knocking out short range correlated nucleons with very high momenta make one more naturally to apply the study of SRCs in the relativistic regime. A relativistic projectile moving along the z-direction probe the light-cone (LC) wave-function of the nucleus, $\psi_{A}(\alpha_{1},k_{1,t},...,\alpha_{i},k_{i,t},...,\alpha_{A},k_{A,t})$, where the LC variable is defined as~\cite{Frankfurt_misak}:
\begin{equation}
  \alpha_{i} = A\left(\frac{E_{i}-p_{i,z}}{E_{A}-p_{A,z}}\right)=A\left(\frac{E_{i}^{lab}-p_{i,z}^{lab}}{M_{A}}\right),
\end{equation}  
where ($E_{i}-p_{i,z}$) and ($E_{A}-p_{A,z}$) are the initial energy and longitudinal momentum of constituent nucleons and the target nucleus, $A$, respectively. $\alpha_{i}$ is invariant under Lorentz boosts in the z-direction. In the rest frame of the nucleus, $E_{A}-p_{A,z}=M_{A}$, where $M_{A}$ is the nuclear mass. 

Similar to the definition of $x_{bj}$ in inelastic scattering (Eq~\ref{xbj_define}), $\alpha_{i}$ denotes the LC fraction of the nucleus momentum carried by the nucleon, hence $\sum_{i}^{A}\alpha_{i}=A$. While $\alpha_{i}\leq 1$ limits the momentum fraction of the nucleon carried by the quark, to have $\alpha_{i}>1$ requires at least two nucleons involved in the scattering. Furthermore, three nucleons are required to share their momentum to have $\alpha_{i}>2$. $\alpha_{i}$ consequently becomes an ideal variable to distinguish between 2N-SRC and 3N-SRC. Considering the energy and momentum conservation law for the nucleon knock-out with a virtual photon from the nucleus, one can rewrite the LC variable as~\cite{src_john}:
\begin{equation}
  \alpha_{i}=x_{bj}\left(1+\frac{2p_{i,z}}{\nu+|\mathbf{q}|}\right)+\frac{W_{N}^{2}-m_{i}^{2}}{2m_{i}\nu},
  \label{alpha_xbj}
\end{equation}
where $\nu$ and $\mathbf{q}$ is the energy and momentum transfer of the virtual photon, respectively, and $W_{N}^{2}=(\mathbf{p_{i}}+\mathbf{q})^{2}$. For the quasi-elastic process, $W_{N}\simeq m_{i}$ yields a simple connection between $\alpha_{i}$ and $x_{bj}$. At sufficiently large $Q^{2}$, $\alpha_{i}$ is usually replaced by $x_{bj}$: 
\begin{equation}
  \alpha_{i}\rightarrow x_{bj}, 
\end{equation}
when $Q_{2}\rightarrow \infty$. However, these two variables have distinct differences for $Q^{2}$ values in few $GeV^{2}$ range. One needs to examine the different scaling of SRCs as a function of $x_{bj}$ and $\alpha_{i}$ at the region of low $Q^{2}$ values. 	
\subsection{Isospin Effect}
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.80\linewidth]{./figures/physics/mom_dis_np}
    \caption[Momentum distribution for proton and neutron and their ratio]{\footnotesize{Left: Momentum distribution for proton (solid) and neutron (dashed) in $^{3}He$; Right: Ratio of proton to neutron momentum distribution. Plots were originally from~\ref{src_john}.}}
    \label{mom_dis_np}
  \end{center}
\end{figure}   
Early analysis assumed the isospin-independence of SRCs, which means that the ratio of neutrons to protons in SRCs is equal to the $N/Z$ ratio of the nucleus. However, numerical studies~\cite{PhysRevC.72.054310} and results from experiments~\cite{Subedi:2008zz} reveal that the tensor interaction dominates the attractive potential of 2N-SRC. Accordingly, one expects that 2N-SRC pairs should be mainly in iso-singlet ($np,~T=0$) states. The iso-triplet ($pp$,$np$ and $nn$, $T=1$) pairs can be close together without interacting strongly until their repulsive forces become strong~\cite{src_john}.

Fig.~\ref{mom_dis_np} shows a calculation of the momentum distribution for protons and neutrons and their ratio in $^{3}He$~\cite{Pieper_Wiringa}. In the assumption of isospin-independence, the momentum ratio of protons to neutrons should be equal to two, but if the SRCs are isospin-dependent, the ratio becomes one when SRCs dominate at $k>k_{F}$. The left plot gives the value of the ratio at $k>k_{F}$ roughly equal to 1.5, which suggests that the isospin effect largely deviates from the assumption of isospin independence. The reason why $np_{T=0}$ configuration does not totally dominates is that the $T=1$ channels are not completely suppressed, especially at very large momentum, where the configuration of 3N-SRC is more complicated. Another calculation~\cite{PhysRevLett.98.132501} extended the study to other nuclei provides the similar results. Shown in Fig.~\ref{isospin_src}, the momentum distribution of $np$ pairs is much more significant than one of the $pp$ pairs at $300<k<600$ $MeV/c$.
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/isospin_src}
    \caption[Isospin effect in momentum distribution]{\footnotesize{Isospin effect in momentum distribution, where lines represents the momentum distribution in $np$ and dots represents the momentum distribution in $pp$. The dip in the $pp$ momentum distribution around 2 $fm^{-1}$ is due to the tensor correlations of protons~\cite{src_john,PhysRevLett.98.132501}.}}
    \label{isospin_src}
  \end{center}
\end{figure} 

The isospin effect in 2N-SRC can be studied by triple-coincidence experiments, which not only measures the scattered electrons and the struck protons in a 2N-SRC configuration but also simultaneously detects protons and neutrons rejected in the opposite direction with equal momentum. Inclusive cross sections is also sensitive to such effect. One can examine the isospin-dependence by measuring the cross section ratio of two isotopes in the SRCs region, such as $^{48}Ca/^{40}Ca$~\cite{e08014_pr} and $^{3}He/^{3}H$~\cite{E12_11_112_pr}.

\section{Probing SRCs}
To isolate the high momentum nucleons and perform clean measurements of SRCs in nuclei, one needs to carefully selecting the proper kinematics settings to suppress other competing processes during scattering. By isolating the process of a high energy probe instantly removing a nucleon from SRCs, one is able to extract reliable information on the spectral function and momentum distribution from the measured observables. 

\subsection{Kinematics Conditions}
Although there are different kinds of reactions for probing SRCs, there share the common kinematic conditions to provide a clean study. Overall, the desire to instantly remove the nucleon from the SRCs can be achieved by requiring sufficiently large energy and momentum transfer scales which significantly exceed the excitation scale of the nucleus~\cite{Frankfurt1981215,Frankfurt_misak}
\begin{equation}
  \nu >> V_{NN}, \qquad |\mathbf{q}| >> m_{N}/c,
  \label{src_condition1}
\end{equation}
where $V_{NN}$ is the characteristic potential of the NN interaction and $m_{N}$ is the nucleon mass. A reaction removing a nucleon from the nucleus under this condition allows the residual system to remain intact, where the spectral function will directly reflect the properties of SRCs~\cite{src_john}.

The contribution of long range interactions, such as MECs, is suppressed by a factor of $Q^{-4}$ with respect to the production of SRCs, and can be generally suppressed by requiring~\cite{M_Sargsian_JPG_29_2003}:
\begin{equation}
  Q^{2} > 1.0~GeV^{2} >> m_{meson}^{2}.
  \label{src_condition2}
\end{equation}
In this condition, intermediate state resonances, such as the isobars current (IC), still have sizeable contributions. For example, for $1~GeV^{2}<Q^{2}<4~GeV^{2}$, $\gamma N\rightarrow \Delta$ transition is comparable with $\gamma N\rightarrow N$. Those resonance states are generally within the region of $0<x_{bj}<1$, and their contributions can be suppressed by working at the region above the quasi-elastic scattering:
\begin{equation}
  x_{bj} > 1.
  \label{src_condition3}
\end{equation}

\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/p_min_x}
    \caption[Minimum momentum of the struck nucleon as function of $x_{bj}$ and $Q^{2}$]{\footnotesize{Minimum momentum of the struck nucleon as function of $x_{bj}$ and $Q^{2}$ for scattering off a nucleon from deuterium (right) and from gold (right), where the values of $Q^{2}$ from bottom to top are 0.5, 1.5, 3.0 and 10 $GeV^{2}$, respectively~\cite{Frankfurt_misak, src_john}. The red line sets the value of the Fermi momentum ($k_{F}$). These plots indicate that heavy nuclei require higher values of $Q^{2}$ and $x_{bj}$ to reach the Fermi momentum and fully suppress the mean field contribution.}}
    \label{kin_cond_q2_xbj}
  \end{center}
\end{figure} 
Fig.~\ref{kin_cond_q2_xbj} demonstrates that the combination of kinematic conditions (Eq~\eqref{src_condition2} and Eq~\eqref{src_condition3}). When $Q^{2}$ value is not sufficiently large ($\sim 0.5~GeV^{2}$) for scattering off nucleons from deuterium, the 2N-SRC production is almost suppressed by other processes even at very higher $x_{bj}$ ($\sim 1.8$). At very high $Q^{2}$ ($\sim 10~GeV^{2}$), the minimum momentum requirement of the struck nucleon easily achieves at relatively low $x_{bj}$ ($\sim 1.3$) due to the highly suppression of mean field effect. For heavy nuclei, the requirement of $x_{bj}$ and $Q^{2}$ is much more strict to reach the Fermi momentum. 

Together with Eq~\eqref{src_condition1}, those kinematic conditions enable the clean measurement of high momentum nucleons from SRCs and meanwhile, largely eliminate the contribution from mean field effect, such as MECs and IC.

\subsection{Inclusive Measurement}
The inclusive cross section measurement of $A(e,e')$ reaction in quasi-elastic region was first applied to isolate SRCs and currently is the only way to probe 3N-SRC. The cross section for $x>1.3$ and $Q^{2}>1~GeV^{2}$ is written as~\cite{Frankfurt1988235}:
\begin{eqnarray}
  \sigma_{A}(x_{bj},Q^{2}) &=& \sum_{j=2}^{A}\frac{A}{j} a_{j}(A) \sigma_{j}(x_{bj},Q^{2}) \nonumber \\
  &=& \frac{A}{2}a_{2}(A)\sigma_{2}(x_{bj},Q^{2})+\frac{A}{3}a_{3}(A)\sigma_{3}(x_{bj},Q^{2})+...,
  \label{xs_src_inclusive}
\end{eqnarray}
where $\sigma_{j}$ is the cross section for scattering from a $j$-nucleon correlation and $a_{j}(A)$ denotes the probability of finding a nucleon in this correlation. First two terms represents the contributions from 2N-SRC and 3N-SRC. 

From Eq~\eqref{2nsrc_mon_scaling} and Eq~\eqref{3nsrc_mon_scaling}, 2N-SRC (3N-SRC) predicts the scaling of the nucleon momentum distribution for heavy nucleus $A$ with respect to the deuterium ($^{3}He$). In the region of $1.3<x_{bj}<2.0$ where 2N-SRC dominates, $a_{2}(A)$ can also be given by the cross section ratio:
\begin{equation}
  a_{2}(A) = \frac{2}{A}\frac{\sigma_{A}(x_{bj},Q^{2})}{\sigma_{D}(x_{bj},Q^{2})},
  \label{src_a2}
\end{equation}
where $\sigma_{D}(x_{bj},Q^{2})$ is the cross section for scattering from the deuterium target. $a_{2}(A)$ is identical to the one defined in Eq~\eqref{2nsrc_mon_scaling} and the formula indicates that at 2N-SRC region, the value of $a_{2}$ is independent of $x_{bj}$ and $Q^{2}$, but only relates to the nuclear number. The value of the ratio on the scaling plateau directly gives the relative number of 2N-SRC pairs in the nucleus.
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/SLAC_2NSRC_First}
    \caption[First evidence of 2N-SRC from SLAC]{\footnotesize{First evidence of 2N-SRC from SLAC~\cite{SLAC_Measurement_PRC.48.2451}. Y-axis is the cross section ratio of $^{56}Fe$ to $^{2}H$ for $Q^{2}=1.2-2.9~GeV^{2}$ and x-axis is $x_{bj}$. The plateau of 2N-SRC clearly is clearly showed at $x_{bj}>1.5$ and agrees with the theoretical prediction based on the 2N-SRC model (lines).}}
    \label{slac_2nsrc_first}
  \end{center}
\end{figure}

Fig.~\ref{slac_2nsrc_first} shows the experiment results from SLAC~\cite{SLAC_Measurement_PRC.48.2451}, which for the first time observed such a plateau using the cross section ratio of $^{56}Fe$ to $^{2}H$ at $x_{bj}>1.5$ and $Q^{2}=1.2-2.9~GeV^{2}$. However, the statistics were limited and the deuterium data were taken at different kinematics, so the result was extracted with nontrivial extrapolations. Recent Jefferson Lab results from Hall-B using Large Acceptance Spectrometer (CLAS)~\cite{PhysRevLett.96.082501} and from E02-019 data in Hall-C~\cite{PhysRevLett.108.092502} studied the values of $a_{2}$ for various nuclei with higher statistics and with better resolution, and both results show sound agreement at the 2N-SRC region (Fig.~\ref{CLAS_2NSRC_3NSRC} and Fig.~\ref{E02019_2NSRC_3NSRC}). 

Similarly, one can study 3N-SRC at $2<x_{bj}<3$ with the cross section ratio of the heavy nucleus to $^{3}He$:
\begin{equation}
  a_{3}(A) = K\cdot\frac{3}{A}\frac{\sigma_{A}(x_{bj},Q^{2})}{\sigma_{^{3}He}(x_{bj},Q^{2})},
  \label{src_a3}
\end{equation}
which is the same as the one in Eq~\eqref{2nsrc_mon_scaling} and denotes the number of $^{3}He$-like 3N-SRC configuration in the nucleus. $K$ is a kinematic constant to correct difference of the electron-proton and electron-neutron cross sections:
\begin{equation}
  K = \frac{\sigma_{ep}+\sigma_{en}}{Z\sigma_{ep}+(A-Z)\sigma_{en}}.
\end{equation}
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/CLAS_2NSRC_3NSRC}
    \caption[2N-SRC and 3N-SRC results from Hall B]{\footnotesize{2N-SRC and 3N-SRC results from Hall B~\cite{PhysRevLett.96.082501}. The top, middle and bottom plots give the cross section ratios of $^{4}He$, $^{12}C$ and $^{56}Fe$ to $^{3}He$, respectively. In each plot, both the 2N-SRC plateau (in $1.5<x_{bj}<2$) and the 3N-SRC plateau (in $x_{bj}>2$) can be observed.}}
    \label{CLAS_2NSRC_3NSRC}
  \end{center}
\end{figure} 

The CLAS data for the first time measured the kinematic region of 3N-SRC and observed the plateau raises at $x_{bj}>2.3$. The E02-019 data, however, yields a different result in this region. From Fig.~\ref{E02019_2NSRC_3NSRC}, the cross section ratio of $^{4}He/^{3}He$ reaches the scaling region slightly later than the CLAS result ($x_{bj}>2.5$). And the scaling plateau can not be conformed due to the large error bars, mainly because of the large statistical subtraction to remove the contamination from the aluminium windows. A simple interpolation of the discrepancy is impossible since two experiments ran at very different $Q^{2}$ range ($Q^{2}\sim 1.6~GeV^{2}$ for CLAS and $Q^{2}\sim 2.7~GeV^{2}$ for E02-019). It is not clear that both measurements were able to isolate the 3N-SRC contributions. The new experiment in Hall-A, E08-014, focuses on studying the scaling of 3N-SRC at $x_{bj}>2$ with much better accuracy, and the new preliminary results will be presented in this thesis. 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/E02019_2NSRC_3NSRC}
    \caption[2N-SRC and 3N-SRC results from E02-019 in Hall C]{\footnotesize{2N-SRC and 3N-SRC results from E02-019 in Hall C~\cite{PhysRevLett.108.092502} comparing with the result from Hall-B, where the blue dots are the E02-019 data and red dots are the CLAS data.}}
    \label{E02019_2NSRC_3NSRC}
  \end{center}
\end{figure} 

The other important study of SRCs in inclusive measurements is the difference of two scaling variables, $x_{bj}$ and $\alpha_{i}$. From Eq~\eqref{alpha_xbj}, the LC variable $\alpha_{i}$ is approximately equal to $x_{bj}$ at large $Q^{2}$. At low $GeV^{2}$, the approximation is not valid and the difference of the scaling behaviour in SRCs as a function of $x_{bj}$ or $\alpha_{i}$ is required to be carefully examined. 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/SLAC_2NSRC_xbj_alpha}
    \caption[Ratio of $^{56}Fe/^{2}H$ as a function of $x_{bj}$ and $\alpha_{2N}$]{\footnotesize{Ratio of $^{56}Fe/^{2}H$ as a function of $x_{bj}$ (left) and $\alpha_{2N}$ (right) for different $Q^{2}$ values~\cite{SLAC_Measurement_PRC.48.2451}, which shows that the LC variable provides better scaling behaviour.}}
    \label{SLAC_2NSRC_xbj_alpha}
  \end{center}
\end{figure} 
Although $\alpha_{i}$ can not be reconstructed in inclusive scattering, one can assume that in PWIA the virtual photon interacts with the nucleon in an 2N-SRC at rest. This assumption leads to a new expression of the LC variable specifically for 2N-SRC:
\begin{equation}
  \alpha_{2N} = 2-\frac{q_{-}+2m}{2m}\frac{\sqrt{W^{2}-4m^{2}}+W}{W},  
\end{equation}
where $q_{-}$ is the initial longitudinal momentum of the struck nucleon and $W^{2}=4m_{N}^{2}+4m_{N}\nu-Q^{2}$. The analysis of SLAC data~\cite{SLAC_Measurement_PRC.48.2451} reveals that $\alpha_{2N}$ can better isolate 2N-SRCs (Fig.~\ref{SLAC_2NSRC_xbj_alpha}) and allows one to examine the transition region from 2N-SRC to 3N-SRC. A more general expression for all $\alpha_{i}$ in the inclusive measurement can be obtained from~\cite{e08014_pr}:
\begin{equation}
  q_{-}\cdot\alpha_{jN}m_{N}+q_{+}\cdot\left(M_{A}-\frac{M_{r}^{2}}{m_{N}(j-\alpha_{jN})}\right)=m_{N}^{2},
\end{equation}
where $j=2,3,...$, $q_{+}$ is the initial transverse momentum of the struck nucleon and $M_{r}$ is the mass of the residual system. Taking $j=3$ can solve for $\alpha_{3N}$ but the exact expression depends on the value of $M_{r}$ since 3N-SRC has much more complicated configuration. As discussed in previous section, 3N-SRC-I is the dominant configuration in 3N-SRC where $M_{r}=2m_{N}$, and give:
\begin{equation}
  \alpha_{3N} = \frac{3}{2}+\frac{1}{2}[\sqrt{ (3+b_{1})^{2}-b_{2}}-b_{1}]
\end{equation} 
where,
\begin{equation}
  b_{1} = \frac{q_{+}}{q_{-}} \frac{M_{A}}{m_{N}}-\frac{m_{N}}{q_{-}},\qquad b_{2} = 16 \frac{q_{+}}{q_{-}}.
\end{equation} 
The value of $M_{r}$ becomes higher for non-parallel configuration, such as 3N-SRC-II. Examining the scaling as a function of $\alpha_{3N}$ and varying the value of $M_{r}$ provides a sensitive probe to the detailed structure of 3N-SRC~\cite{e08014_pr}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Other Experiment Techniques}
\subsection{Semi-Inclusive and Triple-Coincidence Measurements}
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/10yrSRC_fig3}
    \caption[Proton Effective Momentum distribution in $^{3}He$.]{\footnotesize{Proton Effective Momentum distribution in $^{3}He$~\cite{PhysRevLett.94.082305}, where circles and triangles are experimental data in $^{3}He(e,e'p)pn$ three-body break-up and $^{3}He(e,e'p)d$ two-body break-up, respectively. Lines are theoretical calculations from~\cite{Laget200549}. For the missing momentum above the Fermi momentum (250 MeV), the momentum distribution of three-body break-up is much stronger than the one of two-body break-up, indicating the dominance of SRCs in this region.}}
    \label{10yrSRC_fig3}
  \end{center}
\end{figure} 
Proton-knock-out experiments allow the direct access of the proton's initial momentum distribution through the reconstruction of the nuclear spectral function from the exclusive cross sections. In addition to measuring the scattered electron, one can map out the effect of SRCs to the high momentum tail by detecting the struck proton. Since the correlated nucleon in 2N-SRC is ejected on the opposite direction is not detected, one generally treats the $A(e,e'p)$ reaction as semi-inclusive process. 

To evaluate the deviation of a theoretical calculation of the momentum distribution to the experimental cross section, a normalization factor is introduced in Eq~\eqref{quasi_xs_spectral_function} (for only one proton case)~\cite{Higinbotham:2009hi}:
\begin{equation}
  \frac{d^{6}\sigma}{(dEd\Omega)_{e}(dEd\Omega)_{p}} = K\sigma_{ep}S(E_{0},\mathbf{p_{0}})T_{A}(Q^{2}),
\end{equation}
where $K$ is a kinematic factor and the transparency, $T_{A}$ is the probability that a nucleon will be emitted from the nucleus with other effects, such as FSI. Experiments in Hall-C~\cite{PhysRevLett.80.5072,PhysRevC.66.044613,PhysRevC.72.054602} measured the values of $T_{A}$ for several nuclei which were found to be larger than the predictions in IPSM. Such an enhancement is mainly due to the SRCs effect~\cite{Higinbotham:2009hi}. 

Hall-A experiments ~\cite{PhysRevLett.94.082305,PhysRevLett.94.192302} studied the momentum distribution of $^{3}He$ and observed that the strength greatly increases in the high momentum tail compared with the expected strength including SRCs (Fig.~\ref{10yrSRC_fig3}). This scenario is explained as the combination of SRCs and FSI. 

%\subsection{Triple-Coincidence Measurements}
The exclusive cross section measurement of the $A(e,e'pN)$ reaction, or called the triple-coincidence experiment~\cite{PhysRevLett.90.042301,PhysRevLett.99.072501,src_since}, is able to direct probe the scattered electron, the struck nucleon and the spectator nucleon in 2N-SRC. Such an experiment not only can directly conform the production of 2N-SRC, but also can study the types of the nucleon pairs involved in the correlation.  
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/10yrSRC_fig5}
    \caption[Angular correlation between nucleons in 2N-SRC]{\footnotesize{Angular correlation between nucleons in 2N-SRC, where the x-axis is the cosine of the opening angle between the struck nucleon and the spectator nucleon in the $^{12}C(e,e'pp)$ reaction~\cite{PhysRevLett.99.072501}.}}
    \label{triple_src_cos}
  \end{center}
\end{figure} 

A recent experiment in Hall-A, E01-015, ~\cite{PhysRevLett.99.072501,src_since}, has performed such a measurement using electron scattering on carbon target. In the $^{12}C(e,e'pp)$ reaction, the experiment studied the angular correlations between the struck proton and the spectator nucleons. Fig.~\ref{triple_src_cos} gives the distribution of the events in $cos\gamma$ when $p_{m}$=500~MeV/c, which clearly peaks near $cos\gamma=-1$. This result proved that the correlated nucleons are ejected back-to-back from the nucleus. The ratio of $pn$ and $pp$ in 2N-SRC can be extracted by using comparing $^{12}C(e,e'pp)$ and $^{12}C(e,e'pn)$. Fig.~\ref{triple_src_np} shows that the ratio of $np/pp$ pairs is around $18\pm 5$, which conforms that the 2N-SRC is dominated by the two-body tensor interaction. 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,angle=270,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/10yrSRC_fig7}
    \caption[The fraction of $np$ pairs to $pp$ pairs in 2N-SRC]{\footnotesize{The fraction of $np$ pairs to $pp$ pairs in 2N-SRC in carbon from the triple-coincidence experiment in Hall-A~\cite{src_since}.}}
    \label{triple_src_np}
  \end{center}
\end{figure} 

\section{Final State Interaction}
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.80\linewidth]{./figures/physics/FSI}
    \caption[Final state interaction]{\footnotesize{General diagram of final state interaction. The struck nucleon is re-scattered by the $A-1$ system and its final momentum is modified.}}
    \label{fsi}
  \end{center}
\end{figure}
Final State Interaction (FSI) is the effect of the struck nucleon being re-scattered by the $A-1$ recoil system. In PWIA, the nucleons in the nucleus are treated as individual constituents and the space resolution of the electron probe is approximately $1/q$. Hence, in the inclusive cross section measurement at large $Q^{2}$, FSI is negligibly small, based on the fact that the interaction time between the virtual photon and the struck nucleon is significant smaller than the one between the struck nucleon and the recoil system.

However, comparison between the theoretical calculation and experimental results~\cite{PhysRevC.46.1045,PhysRevC.87.024606} shows the violations of y-scaling for heavy target which indicates FSI still plays a significant role in the scattering process even at large $Q^{2}$.
(MORE discussion)

The effect of final state interaction (FSI) is proportional to $1/Q^{2}$. At low $Q^{2}$ the contribution of FSI is large enough to break down the y-scaling feature of quasi-elastic scattering in PWIA~\cite{Day:1987az}. The study of SRCs using inclusive cross section measurement requires sufficient $Q^{2}$ values to eliminate the FSI contribution. The current results of inclusive data (i.e. in Fig.~\ref{SLAC_2NSRC_xbj_alpha}) indicate no dependence of $Q^{2}$ for the scaling region of 2N-SRC, which proves that in the kinematic settings of SRCs study ($Q^{2}>1~GeV^{2}$) FSI has very small contributions.

The argument above is valid since the SRCs configurations are weakly interacting with other components in the nucleus and PWIA in the inclusive measurement is still applicable. However, the contribution of FSI within the SRC may not vanish even at very large $Q^{2}$. When the electron scattering on the nucleon in SRCs, the struck nucleon stays very close to other correlated nucleons and the probability of rescattering from the residual system is large. Despite the possible large contributions, FSI is localized in the SRCs and its contribution can be removed by taking the cross section ratio. For example, the FSI contribution in the 2N-SRC pairs in heavy nuclei should be similar to one in $^{2}H$, and the ratio, $\sigma_{A}/\sigma_{^{2}H}$, should be able to cancel the FSI effect and only yields the clean contribution from 2N-SRC. 

\section{E08014 Experiment}
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/E08014_Kin_Cover}
    \caption[Kinematic Coverage of E08-014 experiment]{\footnotesize{Kinematic Coverage of E08-014 experiment.}}
    \label{kin_cor}
  \end{center}
\end{figure}
An new experiment, E08-014~\cite{e08014_pr}, had been carried out in 2011 in Hall-A at Jefferson Lab, with electron beam energy of $3.356 GeV$ from the continuous electron beam accelerator facility (CEBAF). Utilizing the high resolution spectrometers in their standard configurations, as shown in Fig.~\ref{kin_cor}, this experiment measured the inclusive cross section of $^{2}H$, $^{3}He$, $^{4}He$, and $^{12}C$ at $1.1<Q^{2}<2.5 (GeV/c)^{2}$, which covers the range of $x_{bj}$ from the quasi-elastic peak region to above $3.0$. The absolute cross section results will be used to study the scaling function and momentum distribution at larger missing momentum, as well the effect of FSI. By taking the cross section ratio of heavy targets to $^{2}H$ or $^{3}He$, one can examine the $x_{bj}$ and $Q^{2}$ dependence and SRCs, and measure the values of $a_{2}$ and $a_{3}$. The relatively low $Q^{2}$ setting allows the study of $\alpha_{2N}$ and $\alpha_{3N}$ in the scaling of SRCs. The Calcium isotopes, $^{40}Ca$ and $^{48}Ca$, were also used to study the isospin dependence of 2N- and 3N-SRC. Detailed experiment setup and data analysis will be discussed in this thesis and preliminary results will also be presented. 


==> intro/backup/src_other.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Other Experiment Techniques}
\subsection{Semi-Inclusive Measurements}
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/10yrSRC_fig3}
    \caption[Proton Effective Momentum distribution in $^{3}He$.]{\footnotesize{Proton Effective Momentum distribution in $^{3}He$~\cite{PhysRevLett.94.082305}, where circles and triangles are experimental data in $^{3}He(e,e'p)pn$ three-body break-up and $^{3}He(e,e'p)d$ two-body break-up, respectively. Lines are theoretical calculations from~\cite{Laget200549}. For the missing momentum above the Fermi momentum (250 MeV), the momentum distribution of three-body break-up is much stronger than the one of two-body break-up, indicating the dominance of SRCs in this region.}}
    \label{10yrSRC_fig3}
  \end{center}
\end{figure} 
Proton-knock-out experiments allow the direct access of the proton's initial momentum distribution through the reconstruction of the nuclear spectral function from the exclusive cross sections. In addition to measuring the scattered electron, one can map out the effect of SRCs to the high momentum tail by detecting the struck proton. Since the correlated nucleon in 2N-SRC is ejected on the opposite direction is not detected, one generally treats the $A(e,e'p)$ reaction as semi-inclusive process. 

To evaluate the deviation of a theoretical calculation of the momentum distribution to the experimental cross section, a normalization factor is introduced in Eq~\eqref{quasi_xs_spectral_function} (for only one proton case)~\cite{Higinbotham:2009hi}:
\begin{equation}
  \frac{d^{6}\sigma}{(dEd\Omega)_{e}(dEd\Omega)_{p}} = K\sigma_{ep}S(E_{0},\mathbf{p_{0}})T_{A}(Q^{2}),
\end{equation}
where $K$ is a kinematic factor and the transparency, $T_{A}$ is the probability that a nucleon will be emitted from the nucleus with other effects, such as FSI. Experiments in Hall-C~\cite{PhysRevLett.80.5072,PhysRevC.66.044613,PhysRevC.72.054602} measured the values of $T_{A}$ for several nuclei which were found to be larger than the predictions in IPSM. Such an enhancement is mainly due to the SRCs effect~\cite{Higinbotham:2009hi}. 

Hall-A experiments ~\cite{PhysRevLett.94.082305,PhysRevLett.94.192302} studied the momentum distribution of $^{3}He$ and observed that the strength greatly increases in the high momentum tail compared with the expected strength including SRCs (Fig.~\ref{10yrSRC_fig3}). This scenario is explained as the combination of SRCs and FSI. 

\subsection{Triple-Coincidence Measurements}
The exclusive cross section measurement of the $A(e,e'pN)$ reaction, or called the triple-coincidence experiment~\cite{PhysRevLett.90.042301,PhysRevLett.99.072501,src_since}, is able to direct probe the scattered electron, the struck nucleon and the spectator nucleon in 2N-SRC. Such an experiment not only can directly conform the production of 2N-SRC, but also can study the types of the nucleon pairs involved in the correlation.  
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/10yrSRC_fig5}
    \caption[Angular correlation between nucleons in 2N-SRC]{\footnotesize{Angular correlation between nucleons in 2N-SRC, where the x-axis is the cosine of the opening angle between the struck nucleon and the spectator nucleon in the $^{12}C(e,e'pp)$ reaction~\cite{PhysRevLett.99.072501}.}}
    \label{triple_src_cos}
  \end{center}
\end{figure} 

A recent experiment in Hall-A, E01-015, ~\cite{PhysRevLett.99.072501,src_since}, has performed such a measurement using electron scattering on carbon target. In the $^{12}C(e,e'pp)$ reaction, the experiment studied the angular correlations between the struck proton and the spectator nucleons. Fig.~\ref{triple_src_cos} gives the distribution of the events in $cos\gamma$ when $p_{m}$=500~MeV/c, which clearly peaks near $cos\gamma=-1$. This result proved that the correlated nucleons are ejected back-to-back from the nucleus. The ratio of $pn$ and $pp$ in 2N-SRC can be extracted by using comparing $^{12}C(e,e'pp)$ and $^{12}C(e,e'pn)$. Fig.~\ref{triple_src_np} shows that the ratio of $np/pp$ pairs is around $18\pm 5$, which conforms that the 2N-SRC is dominated by the two-body tensor interaction. 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[type=pdf,angle=270,ext=.pdf,read=.pdf,width=0.60\linewidth]{./figures/physics/10yrSRC_fig7}
    \caption[The fraction of $np$ pairs to $pp$ pairs in 2N-SRC]{\footnotesize{The fraction of $np$ pairs to $pp$ pairs in 2N-SRC in carbon from the triple-coincidence experiment in Hall-A~\cite{src_since}.}}
    \label{triple_src_np}
  \end{center}
\end{figure} 
